Threats Management Throughout the Software Service Life-Cycle

Software services are inevitably exposed to a fluctuating threat picture. Unfortunately, not all threats can be handled only with preventive measures during design and development, but also require adaptive mitigations at runtime. In this paper we describe an approach where we model composite services and threats together, which allows us to create preventive measures at design-time. At runtime, our specification also allows the service runtime environment (SRE) to receive alerts about active threats that we have not handled, and react to these automatically through adaptation of the composite service. A goal-oriented security requirements modelling tool is used to model business-level threats and analyse how they may impact goals. A process flow modelling tool, utilising Business Process Model and Notation (BPMN) and standard error boundary events, allows us to define how threats should be responded to during service execution on a technical level. Throughout the software life-cycle, we maintain threats in a centralised threat repository. Re-use of these threats extends further into monitoring alerts being distributed through a cloud-based messaging service. To demonstrate our approach in practice, we have developed a proof-of-concept service for the Air Traffic Management (ATM) domain. In addition to the design-time activities, we show how this composite service duly adapts itself when a service component is exposed to a threat at runtime.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Kordy, Mauw, and Pieters (Eds.):\\
Graphical Models for Security 2014 (GraMSec'14)\\
EPTCS 148, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.148.1}{10.4204/EPTCS.148.1}}

